GCT-TTE: Graph Convolutional Transformer for Travel Time Estimation

This paper introduces a new transformer-based model for the problem of travel time estimation. The key feature of the proposed GCT-TTE architecture is the utilization of different data modalities capturing different properties of an input path. Along with the extensive study regarding the model configuration, we implemented and evaluated a sufficient number of actual baselines for path-aware and path-blind settings. The conducted computational experiments have confirmed the viability of our pipeline, which outperformed state-of-the-art models on both considered datasets. Additionally, GCT-TTE was deployed as a web service accessible for further experiments with user-defined routes.

==> tables/intersection_based_results.tex <==
    \renewcommand{\arraystretch}{1.5}
    \centering
    \caption{F1-score for intersection-based models}
    \smallskip
    \begin{tabular}{ll|l|l|l|l|l|l}
    \toprule
        Evaluation & OD & Backbone & ACMPS & ACPDS & CNRPark & PKLot & SPKL \\ 
        \midrule
        E$_1$ & FasterRCNN & ResNet & \textbf{0.7527} & 0.7972 & 0.9629 & \textbf{0.9031} & \textbf{0.8848} \\ 
        ~ & ~ & MobileNet & 0.7251 & 0.7636 & 0.9256 & 0.8952 & 0.6195 \\ 
        ~ & ~ & VGG-19 & 0.7282 & 0.7228 & 0.9185 & 0.8951 & 0.8596 \\ 
        ~ & RetinaNet & ResNet & 0.7384 & 0.7856 & \textbf{0.9683} & 0.8313 & 0.8304 \\ 
        ~ & ~ & MobileNet & 0.7069 & 0.7552 & 0.9234 & 0.8125 & 0.7427 \\ 
        ~ & ~ & VGG-19 & 0.7194 & 0.7234 & 0.9126 & 0.7823 & 0.7581 \\ 
        \midrule
        E$_2$ & FasterRCNN & ResNet & 0.5815 & 0.7963 & 0.4728 & 0.7598 & 0.4727 \\ 
        ~ & ~ & MobileNet & 0.5456 & 0.8013 & 0.4253 & 0.7285 & 0.2906 \\ 
        ~ & ~ & VGG-19 & 0.5298 & 0.7857 & 0.4272 & 0.7347 & 0.4792 \\
        ~ & RetinaNet & ResNet & 0.5115 & \textbf{0.9586} & 0.4926 & 0.7736 & 0.7826 \\ 
        ~ & ~ & MobileNet & 0.5267 & 0.9283 & 0.4163 & 0.7561 & 0.7953 \\ 
        ~ & ~ & VGG-19 & 0.4935 & 0.9126 & 0.4012 & 0.7355 & 0.7924 \\ 
        \bottomrule
    \end{tabular}

==> tables/patch_based_results_cnn.tex <==
% divided dataset results
\begin{comment}

\renewcommand{\arraystretch}{1.5}
    
    \centering
    \label{results_table:cnn}
    \caption{F1-score for patch-based methods (convlutional neural network classifiers)}
    \smallskip
    \begin{tabularx}{355px}{XX|X|X|X|X|X|X}
        \toprule
        \multicolumn{2}{l|}{} & ACMPS & ACPDS & CNRPark & PKLot & SPKL & Merged \\
        \midrule
        \multicolumn{2}{l|}{ResNet50} & 0.9968 & 0.9359 & 0.9798 & 0.9955 & 0.8883 & 0.9737 \\
        \multicolumn{2}{l|}{MobileNet} & 0.9992 & 0.9668 & 0.9974 & 0.9995 & 0.9701 & \textbf{0.9991} \\ 
        \multicolumn{2}{l|}{CarNet} & 0.9938 & 0.8765 & 0.9888 & 0.9975 & 0.9542 & 0.9966 \\ 
        \multicolumn{2}{l|}{AlexNet} & 0.9964 & 0.9308 & 0.9920 & 0.9994 & 0.9379 & 0.9937 \\ 
        \multicolumn{2}{l|}{mAlexNet} & 0.9882 & 0.8999 & 0.9870 & 0.9962 & 0.9156 & 0.9898 \\ 
        \multicolumn{2}{l|}{VGG-16} & 0.9929 & 0.9346 & 0.9933 & 0.9990 & 0.9343 & 0.9952 \\ 
        \multicolumn{2}{l|}{VGG-19} & 0.9941 & 0.9593 & 0.9917 & 0.9991 & 0.9222 & 0.9966 \\ 
        \multicolumn{2}{l|}{CFEN} & 0.9886 & 0.9098 & 0.9845 & 0.9971 & 0.9156 & 0.9924 \\ 
        \midrule
        \multicolumn{2}{l|}{EfficientNet-B0} &\textbf{0.9952} & \textbf{0.9950} & \textbf{0.9952} & \textbf{0.9254} & \textbf{0.9795} & \textbf{0.9986} \\ 
        \multicolumn{2}{l|}{EfficientNet-P} &\textbf{ 0.9992} & \textbf{0.9866} & \textbf{0.9991} & \textbf{0.9995} & \textbf{0.9795} & \textbf{0.9986} \\ 
        \bottomrule
    \end{tabularx}

\end{comment}

% merged dataset results

\renewcommand{\arraystretch}{1.5}
    
    \centering
    \label{results_table:cnn}
    \caption{F1-score for patch-based methods (convlutional neural network classifiers)}
    \smallskip
    \begin{tabularx}{355px}{XX|X|X|X|X|X}
        \toprule
        \multicolumn{2}{l|}{} & ACMPS & ACPDS & CNRPark & PKLot & SPKL\\
        \midrule
        \multicolumn{2}{l|}{ResNet50} & 0.9379 & 0.8407 & 0.9380 & 0.9926 & 0.6674 \\
        \multicolumn{2}{l|}{MobileNet} & 0.9971 & \textbf{0.9343} & 0.9663 & 0.9991 & 0.6910 \\ 
        \multicolumn{2}{l|}{CarNet} & 0.9882 & 0.8377 & 0.9332 & 0.9984 & 0.7131 \\ 
        \multicolumn{2}{l|}{AlexNet} & 0.9914 & 0.8820 & 0.9555 & 0.9990 & 0.7132 \\ 
        \multicolumn{2}{l|}{mAlexNet} & 0.9813 & 0.8577 & 0.9176 & 0.9959 & 0.6937 \\ 
        \multicolumn{2}{l|}{VGG-16} & 0.9923 & 0.8936 & 0.9496 & 0.9985 & 0.5700 \\ 
        \multicolumn{2}{l|}{VGG-19} & 0.9877 & 0.9152 & 0.9629 & 0.9988 & 0.6801 \\ 
        \multicolumn{2}{l|}{CFEN} & 0.9829 & 0.8302 & 0.8482 & 0.9966 & 0.5367 \\ 
        \midrule
        \multicolumn{2}{l|}{EfficientNet-B0} & 0.9950 & 0.9259 & 0.9572 & 0.9993 & 0.7330 \\ 
        \multicolumn{2}{l|}{EfficientNet-P} & \textbf{0.9982} & 0.9125 & \textbf{0.9683} & \textbf{0.9995} & \textbf{0.7393} \\ 
        \bottomrule
    \end{tabularx}

==> tables/patch_based_results_vt.tex <==
% divided dataset results
\begin{comment} 
 \renewcommand{\arraystretch}{1.5}
    
    \centering
    \label{results_table:vt}
    \caption{F1-score for patch-based methods (vision transformer classifiers)}
    \smallskip
    \begin{tabularx}{355px}{XX|X|X|X|X|X|X}
        \toprule
        \multicolumn{2}{l|}{} & ACMPS & ACPDS & CNRPark & PKLot & SPKL & Merged \\ 
        \midrule
        \multicolumn{2}{l|}{ViT (no prt)} & 0.9806 & 0.8966 & \textbf{0.9881} & 0.9844 & 0.8727 & 0.9884 \\ 
        \multicolumn{2}{l|}{ViT (prt)} & 0.9595 & \textbf{0.9370} & 0.9845 & \textbf{0.9983} & \textbf{0.9383} & 0.9822 \\ 
        \multicolumn{2}{l|}{DeiT (prt)} & 0.9542 & 0.9201 & 0.9833 & 0.9880 & 0.9027 & \textbf{0.9915} \\ 
        \multicolumn{2}{l|}{PiT (prt)} & 0.9294 & 0.9372 & 0.9451 & 0.9740 & 0.9333 & 0.9584 \\ 
        \multicolumn{2}{l|}{ViT (SPT LSA)} & \textbf{0.9935} & 0.9073 & 0.9804 & 0.9967 & 0.9320 & 0.9410 \\ 
        \bottomrule
    \end{tabularx}

\end{comment}

% merged dataset results
\renewcommand{\arraystretch}{1.5}

\centering
\label{results_table:vt}
\caption{F1-score for patch-based methods (vision transformer classifiers)}
\smallskip
\begin{tabularx}{355px}{XX|X|X|X|X|X}
    \toprule
    \multicolumn{2}{l|}{} & ACMPS & ACPDS & CNRPark & PKLot & SPKL \\ 
    \midrule
    \multicolumn{2}{l|}{ViT} & 0.9789 & 0.8152 & \textbf{0.9193} & \textbf{0.9966} & 0.7335 \\ 
    \multicolumn{2}{l|}{ViT (SPT LSA)} & 0.9339 & 0.8055 & 0.9179 & 0.9906 & 0.7412 \\ 
    \multicolumn{2}{l|}{ViT (pre-trained)} & \textbf{0.9856} & \textbf{0.8263} & 0.9083 & 0.9856 & 0.6600 \\
    \multicolumn{2}{l|}{DeiT (pre-trained)} & 0.9556 & 0.8209 & 0.8902 & 0.9928 & 0.7010 \\ 
    \multicolumn{2}{l|}{PiT (pre-trained)} & 0.9334 & 0.7122 & 0.9084 & 0.9818  & \textbf{0.7455} \\ 
    \bottomrule
\end{tabularx}
